Database Theory + X: Database Visualization

We draw a connection between data modeling and visualization, namely that a visualization specification defines a mapping from database constraints to visual representations of those constraints. Using this formalism, we show how many visualization design decisions are, in fact, data modeling choices and extend data visualization from single-dataset visualizations to database visualization

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> content/fkeys.tex <==


\subsection{Mapping Foreign-key Constraints}

Foreign key constraints are used extensively to model network and hierarchical data.  For instance, the former is modeled as node and edges tables as in \Cref{fig:foreignattrgraph}, while the latter is modeled as a single nodes table $N(\underline{id}, parent, \dots)$ with a constraint $C(N.parent,\underline{N.id})$.  We thus draw on existing visual metaphors from network~\cite{gibson2013survey}, hierarchical~\cite{schulz2010design,bruls2000squarified} (e.g., treemaps), and multi-view
%, and parallel coordinate
visualizations to propose methods to visually map a foreign key constraint $C(S.X, T.Y)$.  

We categorize the visualization designs into two classes: {\it explicit} if they render marks to encode the relationship, and {\it implicit} otherwise.
For instance, network visualizations render each node as a mark and the relationship between two nodes using an explicit link; the spatial placement of the node marks is based on various layout algorithms.   In contrast, treemaps use spatial containment to render parent-child relationships by subdividing a parent's spatial extent to render its children.  Finally, multi-view visualizations use shared scales and alignment to denote common attributes across multiple views.

%parallel coordinate designs treat each attribute as a separate table that is rendered as a separate view, and draws links between them to denote that they are from the same table.  
% if they rely on spatial positioning or shared scales.  
The same way a data attribute can be encoded in more than one visual channels,    a relationship may be expressed using a combination of explicit and implicit methods.  Furthermore, just as new visualization designs continue to be discovered, we do not claim the designs below are exhaustive; they simply represent a set of simple designs.  Below, we will assume that $S$ and $T$ each have a single mark table $V_S$ and $V_T$.


\subsubsection{Explicit Representation: Marks.}

What does it mean to render a constraint in the visualization?
Tables are populated with rows to instantiate marks and values to set  mark properties, 
but a foreign key constraint $C(S.X,T.Y)$ is an abstract logical statement about data. 
A naive approach might instantiate $C$ as a table $T_C(X,Y)$ and then render it as a single-table visualization.  Although syntactically correct, it is semantically nonsensical because $S.X=T.Y$ for every row in $T_C$.  

%    \forall s\in S \exists t\in T,\ s.X = t.Y

Foreign attributes (\Cref{ss:joins}) provide a powerful way to enforce foreign key constraints in the visualization by simply referencing them in the visualization mapping.     
The most direct way is to treat $C$ as a table in the naive approach, but map functions $f_1(S.X)$ and $f_2(T.Y)$ to mark properties. 

\begin{example}
For the following hierarchical dataset, we render nodes as points ($V_N$) and links from child to parent nodes ($V_{E_1}$) because the spatial position of the point mark is a key (\Cref{ss:mapkeys}).  The specific positions of the points do not matter, so its specification is denoted with ``$\dots$''.
\begin{align*}
      &N(id, p),  C(N.p, \underline{N.id})\\
V_N = &\{ N\to point, \dots \}\\
V_{E_1} = &\{ C\to link, V_N[id].(x,y)\to (x1,y1), V_N[p].(x,y)\to (x2,y2) \}
\end{align*}
\end{example}
%
It is not necessary to render the constraint as a line between marks.  It is sufficient for $f_1(S.X)$ and $f_2(T.Y)$ to return keys (e.g., $N.id$, $V_N.(x,y)$) that are (1) mapped to the same mark's properties, and (2) those keys are present as data attributes or channels in $V_S$ and $V_T$, respectively.   
For instance, the following renders the foreign key constraint using a label instead:
%, and is valid if $V_N$ labels the points with the corresponding node $id$:
%For example, we could have defined the links by mapping from the nodes table $N$ instead.   From $N$, both sides of the foreign key constraint $C$ are accessible, and can be used to specify the start (via $V_N[N.p]$) and end (via $V_N[N.id]$) of the link.
%%
%\begin{align*}
%V_{E_2} = &\{ N\to link, V_N[p].(x,y)\to(x1,y1), V_N[id].(x,y)\to (x2,y2)\}
%\end{align*}
%
%There is no restriction on the type of mark that is needed to enforce a foreign key constraint.
%
\begin{example}\label{ex:explicit-labels}
Table $T$ contains a set of entities, $S$ contains the corresponding names of the entities, and there is a 1-1 relationship between $T$ and $S$.
We wish to render $T$ as points, and label each point with its name:
\begin{align*}
    &T(\underline{id}, a, b), S(\underline{id}, name), C(\underline{S.id}, \underline{T.id})\\
    V_T =& \{T\to point, a\to x, b\to y \}\\
    V_S =& \{S\to text, name\to text, 10\to dx, V_T[c].(x,y)\to (x,y)\}
\end{align*}    
Notice that $V_T[c].(x,y)$ is a key of both $S$ and $T$ because $V_T.(x,y)$ is a key and there are 1-1 relationships between $V_T$, $T$, and $S$.   
\end{example}

%
%\begin{align*}
%    M = \{ C\to marktype, \dots, f_1(S.X)\to A_1, f_2(T.Y)\to A_2 \}
%\end{align*}
%
%\begin{example}
%    The node-link visualization (\Cref{ex:nodelinkfkey}) draws links 
%\end{example}
%
Since the main requirement is that the relationship's keys are mapped to properties of the same mark, the specific channel they are mapped to does not technically matter (though some channels may be more effective than others).   

\begin{example}
Using the same dataset as \Cref{ex:explicit-labels}, we render $T$ as labels of the $id$ attribute and $S$ as a list of names positioned by $id$.   We instead render $C$ as a list of strings: each string is formatted to render the ids of the related entities. 
\begin{align*}
    V_T =& \{ T\to label, id\to text, a\to x, b\to y\}\\
    V_S =& \{ S\to label, name\to text, 0\to x, id\to y\}\\
    V_C = &\{ C\to text, 
    f"\texttt{\{}T.id\texttt{\}=\{}S.id\texttt{\}}"\to text,
    id\to y, 10\to x \}
\end{align*}    
Note that because we are treating $C$ as a table, $id\to y$ refers to $id^{th}$ relationship:
\end{example}


%The following renders a line between marks in $M_T$ and $M_S$ that have a foreign key relationship as defined by $C$.
%\begin{align*}
    %\{ C\to line, M_T[C.X].(x,y)\to (xs,ys), M_S[C.Y].(x,y)\to (xe,ye) \}
%\end{align*}


\subsubsection{Implicit Representation: Spatial Nesting}

The major drawback of the explicit representation is that marks occupy the limited rendering region of the visualization.  This can easily lead to overcrowding or overlapping marks, which then violate the key constraints that the visualization needs to preserve.  For this reason, an alternative is to use spatial organization to implicitly denote relationships.   We start with spatial nesting, which is used to denote N-1 relationships common in hierarchical data.  This is exemplified by small-multiples, facetting, treemaps, and other nested visualization designs~\cite{hive,bruls2000squarified}.

The key abstraction is that the parent entities in the relationship (the 1 side of the N-1 relationship) map to marks whose spatial extents are now the canvases that the child entities for whom they have a relationship are drawn within.  

\begin{example}
The following database contains annual price information for stores ($S$) and their latitude-longitude locations ($L$).  There is a N-1 relationship between $S$ and $L$.   $V_L$ renders $50\times50$ rectangles at each store location, and $V_S$ renders the price data as a scatterplot.   Mapping the constraint $C\to nest$ specifies that only the $S$ rows for a given store should be rendered within the extent of its related mark in $V_L$.
\begin{align*}
    &L(id, lat, lon), S(id, cid, year, price), C(S.cid, \underline{L.id})\\
    V_{L} =& \{L\to rect, lat\to x, lon\to y, 50\to w, 50\to h\} \\
    V_{S} =& \{S\to point, year\to x, price\to y\} \\
    &\{C\to nest\}
\end{align*}
\end{example}
%
%Here, the width and height of the marks in $V_T$ are constants and known ahead of time.   In cases where we don't know the spatial extent of the containers because they are computed by a layout algorithm or determined by the marks in $V_S$.  This requires flexible support for layout, which we defer to \Cref{ss:layout}.


From this perspective, a multi-view visualization is simply an application of spatial nesting.  There is a root table containing a single row that maps to the visualization's spatial extent.  All other tables have a N-1 relationship with the root table, and are spatially nested within its mark.  

\subsubsection{Implicit Representation: Shared Scales \& Alignment}

Although nesting is applicable for N-1 relationships, it is less suitable for N-M or 1-1 relationships.  In these cases, a common alternative is to share axes and possibly also alignment.  Returning to the constraint $C(S.X, T.Y)$, let the two tables be mapped to marks as follows, where a function of each table's key is mapped to some spatial channel $c$:
\begin{align*}
    V_S &= \{ S\to \dots, f_S(X) \overset{s_S}{\to} c_S\}\\
    V_T &= \{ T\to \dots, f_T(Y) \overset{s_T}{\to} c_T\}\\
\end{align*}
%
Recall that the definition of a foreign key is that $S.X$ and $T.Y$ share their attribute domains.  Thus, a sufficient way to map this is to ensure that the domains of their scaling functions $s_S$ and $s_T$ are the same: $s_S.domain = s_T.domain$. 
Concretely, we illustrate the following visualization in \Cref{fig:implicit-align}(a), which renders $S$ and $T$ as labels.
We include the ids in \grey{grey} and label each table for reference.
Since the scales have the same domain, the rows are consistently ordered---it is technically possible, but difficult, to relate the $i^{th}$ rows from $S$ and $T$.
\begin{align*}
    & T(\underline{id}, t), S(\underline{id}, s), C(\underline{S.id}, \underline{T.id})\\
V_S =& \{S\to label, id\overset{s_S}{\to} y, 0\to x, t\to text  \}\\
V_T =& \{T\to label, 0\to y, id\overset{s_T}{\to} x, s\to text  \}
\end{align*}
%

Each of the following methods shows how this foreign key relationship can be visually reinforced.  Each method builds on the previous, and is respectively shown in \Cref{fig:implicit-align}(b-e):
\begin{enumerate}
    \item \stitle{Relative Alignment} guarantees that the mark is consistently ordered and relatively positioned within both views by enforcing that the ranges of the scale functions are also the same: $s_S.range = s_T.range$.   
    \item \stitle{Shared Channel} requires that the spatial channels are the same $c_S=c_T$.  In the example, $S.id$ and $T.id$ are both mapped to the y spatial channel.
    \item \stitle{Absolute Alignment} ensures that the spatial extents of the views $V_S$ and $V_T$ are aligned along the shared channel $c_S=c_T$ ($y$ in the example).
    \item \stitle{Spatial Proximity} ensures that the shared channels are positioned near each other to reduce separation effects~\cite{talbot2014four}.
\end{enumerate}
% 
\begin{figure}
    \centering
    \includegraphics[width=.9\columnwidth]{figs/implicit-align.pdf}
    \vspace{-.2in}
    \caption{Foreign key relationship between $S$ and $T$ is preserved by (a) shared scale domains, and can be progressively reinforced by (b) shared scale ranges, (c) shared channels, (d) absolutely alginment of the views, and (e) spatial proximity.  }
    \label{fig:implicit-align}
\end{figure}


==> content/grammar.tex <==

\subsubsection{Overview}

We will first describe the full grammar, and then introduce syntactic sugar to simplify how common cases are specific.

The grammar is almost identical to a standard single table grammar.  A plot consists of data transformations applied to the database along with definitions for one or more views, where each view is defined by a data source, mark type, visual mappings, and scales.   A scale can be shared across multiple views, and the visual mappings map an expression over the data source to a mark attribute.

The grammar differs in several ways.
First, a data source can be a table or constraint.  If it is a table, the expressions must be over data attributes in the table.  If it is a constraint, then expressions may reference attributes from either table,  marks in views where either table is a data source, or the mark attributes.     
Second, a foreign key constraint can rendered using a {\it containment} mark type, in which T1 is as a subplot within T2's marks.
Third, the grammar provides a flexible way to assign mark attributes based on layout algorithms.  An expression can also be a layout algorithm, which is evaluated over a partially rendered view where nonlayout mark attributes have been calculated, and can run arbitrary algorithms to assign the remaining mark attribute values.  

\begin{verbatim}
    P := ( V: views*, transform: t* )
    V := ( data: d, mark: t, mapping: m, scales: s )
    data := table | constraint
    mapping := { vname: e }*
    scales := { vname: scale }*
    transform := operator(table; params)
    e := attr | `markof(` attr `)` ("." attname)? | layout 
    layout := "auto()" | "equi()" | ... 
    transform := operator*
    operator := filter | project | join | ...
    constraint := attr '=' attr
    attr := tablename "." attname
    mark := point | line | ... | containment
    tablename := string
    attname := string
    vname := string
\end{verbatim}


\begin{itemize}
    \item Each table maps to a mark type, such that each row is rendered as a separate mark of that type.  
    \item An attribute domain is rendered as an axis 
    \item Foreign Key references are visually represented
\end{itemize}

\subsubsection{Visualization Concepts}

A visualization draws a collection of marks and axis objects on a canvas.   A mark defines a set of visual attributes and can be spatially rendered on the canvas.  We support the standard point, square, rectangle, bar, and line marks; the square and rectangle can be treated as canvases, which enables recursively defined visualizations.   Analogous to a data attribute domain, each visual attribute has a range (e.g., spatial range, color range, etc).  An axis renders a scaling function from an attribute domain to a visual range.

Scales.


==> content/impl.tex <==
\section{Implementation}\label{s:impl}


We implement our formalism as \sys, a compact Javascript library that .
Programs written with the library can be (de)serialized as JSON specifications for portability.



==> content/layout.tex <==

\begin{figure*}[htb]
    \centering
    \includegraphics[width=.9\textwidth]{figs/scales.pdf}
    \caption{\sys layout functions generalize scales by decoupling the steps---layouts can be trained and applied to different data. (a) The shared scale s is initialized with the values of $S.b$ and $T.d$ to train its domain, and then applied to the same attributes to derive their mark properties.   (b)   }
    \label{fig:scales}
\end{figure*}


\subsection{Layouts}
\label{ss:layout}

At its core, a data visualization spatially organizes marks in a way that is faithful to patterns in the data (i.e., preserves the database constraints), and a graphical grammar is a flexible way to specify the mark layout as a function of data.   
In a sense, part of the grammar's purpose is to define a layout algorithm, and although existing graphical grammars do not support arbitrary layout algorithms, they already support a specialized type: scaling functions.

This subsection first reframes scaling functions as a limited type of layout algorithm that translates scalar data values to spatial channel values, and then generalizes the concept to more expressive layout algorithms. We then extend our formalism to support arbitrary layout algorithms.  


\subsubsection{Scales as Layout}

\Cref{fig:scales}(a) illustrates how a scale function $s$ is used in existing grammars to map $S.b\to y$ in $V_S$ and $T.d\to y$ in $V_T$. The training phase reads $S.b$ and $T.d$ values to determine the attribute's domain.  The apply phase then independently evaluates $s$ on each value of $S.b$ and $T.d$ to produce a $y$ value. 
%
Scales are layout functions that are restricted along three dimensions.   The inputs to the training phase are restricted to the mapped data attributes (e.g., $S.b$, $T.d$), they emit a value for a single visual channel, and their scope is limited to the value of a single mark property.   For instance, $s$ maps the first $b$ value in $S$ (4)  to the y alue $80$ in $V_S$.   

In contrast, layout algorithms require more expressive power along all three dimensions.
Consider the force-directed layout $l_{fd}$ used to render the node-link visualization in \Cref{fig:scales}(b).   The layout algorithm is trained on the edges table yet applied to compute positions for node marks. Further, every node position consists of multiple visual channels ($x,y$) and depends on the positions of the other nodes, so the scope of the algorithm is all of the (partially rendered) marks in the view.
%Since layout algorithms operate in the pixel space, they may also need access to the spatial positions of related marks.



\subsubsection{A Formalism for Layout Algorithms}

A layout algorithm is initialized with the marks table of the view it is applied to, as well as one or more tables that adhere to a pre-defined schema (including foreign key constraints).
For instance, a force-directed layout algorithm that is sensitive to the node size expects inputs with following the schema, where $V$ is the table of node marks with a spatial extent ($w,h$) and $E$ is the set of edges:
%
$$E(sid,tid), V(\underline{id},w,h), C(E.sid,\underline{N.id}), C(E.tid,\underline{N.id}).$$
%
In contrast, a label placement algorithm expects a set of node marks with the positions and spatial extents of the labels: 
$$V(\underline{id},w,h,x,y)$$
%
The input tables are simply passed in during layout initialization,
and the algorithm is referenced in the same way as a scales function to derive one or more visual channels.  
For instance, the following passes in the ids of the start and end nodes in the $Edges$ table as $E$, and the id, width, and height from the node marks table $V_N$ as $V$\footnote{  If $l_{fd}$ is only used in one view, the marks table will be automatically passed in if it is omitted.
}.
%
\begin{align*}
    l_{fd} = & force(Edges.(s,t), V_N.(id,w,h))\\
    V_N = & \{ T\to point,  price\to r, \square\overset{l_{fd}}{\to}(x,y)\}
\end{align*}
% 
The layout can be initialized with the marks table because the algorithm is run after initially allocating the marks and computing all properties that are independent of the layout algorithm.  

The main constraint is that there must be a path of foreign key relationships (of any arity) between the views that reference the layout (e.g., $V_N$) and the tables that it is initialized with ($Edge,V_N$).  The intuition is that the spatial positions of a view's marks is determined by its underlying data data, as well as any related data or mark tables---data that is unrelated should not have an effect.  
For instance, the positions of nodes in a node-link view are dependent on the node sizes (mark properties), the edges table (related tables), and the view's spatial extent (dependent on its spatial nesting). 

The left-hand side of a mapping that references a layout algorithm is always empty ($\square$).  Although the notation $\overset{l}{\to}$ emphasizes that layout is a mapping from data to pixel space, it is also cumbersome.  We simplify the notation by inlining the layout initialization on the left-hand side, so the above example can be rewritten as:
%
$$ V_N = \{ T\to point, price\to r, layout(Edges.(s,t))\to(x,y)\}$$
%



\subsubsection{Examples}

We start visualizations of a hierarchical dataset, where each node in $N$ references its parent: $N(\underline{id}, a, pid), C(N.pid,\underline{N.id})$.   We omit the view definition for the edges because they are the same as the node-link diagrams throughout the paper.  

The first visualization is a tree layout using an algorithm that only considers the set of edges.  The node positions are dependent on all nodes in the hierarchy, so we define it as:
$$V_N = \{ N\to point, 10\to r, tree((id,pid))\to(x,y) \}$$
%
Another common design is a treemap, where each layer of nodes is spatially nested within its parent's spatial extent.   The following renders two layers using squarify~\cite{bruls2000squarified} algorithm:
\begin{align*} 
&T_1(id,a), T_2(id,pid,b), C(T_2.pid,\underline{T1.id})\\
V_1 = &\{T_1\to rect, squarify(a)\to(x,y,w,h), `red'\to color\}\\
V_2 = &\{T_2\to rect, squarify(b)\to(x,y,w,h), `blue'\to color\}\\
%V_3 = &\{T_3\to rect, squarify(c)\to(x,y,w,h), `white'\to color\}\\
& \{ C\to nest \}
\end{align*}
%
%Suppose we wish to render 
%\begin{align*}
%    V_P = \{  sum(V_C[id].h)+10\to h  \}\\
%    V_C = \{ id\to  \}
%\end{align*}
%
The final example avoids label overlap.  Here, the layout placement algorithm is initialized with attributes from two different tables $V_N$ (which have the initial label positions) and $V_L$ (when partially rendered, knows each label's size).  This is well-defined because the two tables have a 1-1 relationship and share the same key:
\begin{align*}
& T(\underline{id}, a,b,text)\\
V_N = & \{ T\to point, a\to x, b\to y \}\\
l =& placement((V_L.id,V_N.x,V_N.y,V_L.w,V_L.h))\\
V_L = & \{ T\to label, text\to text, l\to (x,y) \}
\end{align*}




\subsection{Automatic Layout}

We have established that
* layout algorithms map nothing to mark properties
* views are marks that other table are nested within
* there is a root rectangle (the canvas) for which all other views are nested within



==> content/operators.tex <==

\section{Transformations}\label{s:transforms}

\subsubsection{Joins}

Join is a fundamental operator in relational algebra, and the theoretical foundation of relational languages such as SQL.  Denoted $\bowtie(R,S;A)$, it matches records in table $R$ with records in table $S$ if they have the same value for attributes $A$.  This is equivalent to \texttt{SELECT * FROM R, S WHERE R.A = S.A} in SQL.   


\subsubsection{Decomposition}

One of the goals of relational data modeling is to identify a normal form that reduces data redundancy.   Informally, redundancy occurs when the same logical information is stored multiple times in a table.  In a database, this can waste storage and more importantly, can lead to data errors if the contents of the duplicates diverge under database updates.  In a visualization, redundancy can lead to visual clutter as well as misinterpretations of the data.

The first decomposition operator $\Upsilon(T,A_R,A_S)$
replaces $T(A_T)$ with tables $R(A_R)$ and $S(A_S)$, where  $A_T = A_R\cup A_S$ and $A_{\cap}=A_R\cap A_S$.   Unfortunately, most decompositions are lossy because joining $R$ and $S$ may produce spurious rows not found in $T$.  A correct (lossless) decomposition is one where 
$T = R\bowtie_{A_{\cap}} S$.  This is guaranteed if $A_{\cap}$ is a key of $T_R$ or $T_S$.

The second decomposition operator $\upsilon(T,A)$ where $A\subset A_T$ replaces $T(A_T)$ with tables $R(A)$ and $S(rid,A_T-A)$, where $S.rid\to R.id$.   This in essence eliminates duplicates of $A$ by storing them in a separate table, so that $S$ only contains references to $R$'s id.

%\begin{figure}
%    \centering
%    \includegraphics[width=\columnwidth]{figs/ex-normalize.pdf}
%    \caption{Data normalization changes the resulting visual forms.}
%    \label{fig:ex-normalize}
%\end{figure}
%

\subsubsection{Projection}

$\pi(T; e_1\to name_1,\dots,e_n\to name_n)$

\subsubsection{Filter}

$\sigma(T; p)$



==> content/related.tex <==
\subsection{Related Work}


Keim's VisDB uses different visualization and data mining techniques to visualize a single table in a way that helps users identify useful patterns such as functional dependencies.  In contrast, \sys is a formalism to map constraints such as functional dependencies to their visual forms.

A long line of work in the data management community has focused on identifying functional dependencies, such as CORDS. 

\subsection{Graphical Grammars}


\ewu{example}

%Because of this, features such as aggregation, grouping, and faceting implicitly assume additional structure over the input table that requires custom grammar operators and concepts to handle.  

%However, if this structure were encoded in a multi-table database, then they (as well as other visualizations) can be easily expressed using a compact set of grammar constructs.  

\subsection{Specialized Visualization Designs}


An exception are specialized grammars.  For instance,  HiDe is specifically for space filling visualizations, where hierarchical relationships explicit in the visualization specification.

In this paper, we argue that a reason is that such visualizations are of multiple tables!

\subsection{Graph Visualizations}

\subsection{Tree Visualizations}

Survey of tree visualizations
http://cluster.cis.drexel.edu/~cchen/ivs/sample.pdf

five major visualization types

* node link: tree
* nested enclosed layout.  when parent's "area" subsumes child's
* adjacency layout/icicle.   maps to horizontal length axis
* indentation.   emphasizes hierarchical relationships, but everything else is fixed
* matrix. matrix is bad for hierarchical relationships because it is not faithful to the desired data model!

